Sensing and Communication with Quantum Microwaves

The thesis establishes a link between theoretical foundations and practical applications in the emerging field of propagating quantum microwaves. Although the concrete focus of the main results lies in specific quantum communication and sensing protocols, the thesis also gives a self-contained introduction to quantum parameter estimation and Gaussian quantum continuous variables, justifying the theoretical results used. Motivated, firstly, by the compatibility between superconducting circuits (a promising quantum computing platform), and the microwave frequency range; and, secondly, by the transparency window of the atmosphere to these frequencies, the work contains two concrete contributions to the fields of microwave quantum sensing and communication: a novel protocol that uses frequency entanglement to measure the first order dependence in frequency of the reflectivity of an object; and a large investigation on different aspects of entanglement degradation due to loss and atmospheric absorption in the context of continuous-variable entanglement distribution for the task of quantum teleportation in open-air. The dissertation includes, as a last chapter, an article that reviews the state-of-the-art in quantum microwave technology, and proposes different research lines, including quantum communication between Earth-based stations and satellites, quantum radar, direct dark matter detection, and exploration of the quantum properties of the cosmic microwave background. This more speculative, yet rigorous chapter closes with a roadmap for possible future research lines in the field of propagating quantum microwaves, that can serve as an outlook of the thesis.

==> abstract/abstract-Long.tex <==
%!TEX root = ../dissertation.tex

\begin{otherlanguage}{portuguese}
\begin{abstract}
\abstractPortuguesePageNumber

Quantum mechanics is a physical theory that has benefited enormously from the mathematics community. On the one hand, the group-theoretic formulation of Hilbert, Weyl and others, has helped refine the rigor, clarifying some concepts; on the other, and more recently, quantum mechanics has started to take ideas from information theory through the work by Shannon, Fisher, and others. Taking a pragmatic approach, and assuming a `peaceful coexistence' between quantum mechanics and relativity, we can say that once the main predictions of quantum mechanics are experimentally demonstrated, in particular the existence of beyond-classical correlations between bipartite systems, the theory can then be put to \textit{use}. More specifically, rigor and an information-oriented perspective, combined, produce a theory that is robust, and that can start to leave the proof-of-principle experimental status into the realm of applicability. It is at this point that quantum \textit{technology} enters the play: Industry starts to show interest in the quantum world, in a battle to capitalize the results from the last hundred years, with the goal of solving real-life problems with the new tools available, sometimes with a hyped approach that only time, together with more foundational work, will prove opportunistic.

Quantum technologies are typically applied to three categories: computation,  communication, and sensing. Industrial and political interest is justified: quantum computation has an enormous potential,  not only in the promise of faster-than-classical, efficient computation, but also for simulating quantum systems; quantum communication could bring unprecedented security due to its inherent sensitivity
   towards eavesdropping, creating interest from the banking community. Some of its protocols will have to be incorporated in the 
   quantum internet; and quantum sensing, which goes beyond any classically-achievable resolution, promises sci-fi-like
    ideas as quantum radar, direct detection of dark matter, or exploring the quantum properties of the cosmic microwave background.

In this thesis we give our theoretical contribution to one such emerging quantum technology: propagating quantum microwaves. This platform  finds its most direct motivation in the fact that superconducting circuits, one of the most promising quantum computing platforms, which operate at cryogenic (millikelvin), emit radiation that fits in the GHz window.  Therefore, if one wishes to set up 
 a communication network between such chips, it makes sense to be able to have a technology toolbox that is able to exploit 
 the quantumness of these propagating fields. Moreover, the atmospheric transparency window for microwave frequencies makes 
 them suitable candidates for other tasks, such as quantum communication between Earth-based stations and satellites, or for 
 sensing, including, but not limited to, quantum radar, or imaging. Recent advances in microwave-dedicated photocounters 
 encourages us more to investigate this relatively new research field, as counting photons out of an electromagnetic field 
 is one of the key aspects of any quantum-related protocol, be it in communication or in sensing.

The first part of the thesis is devoted to setting a sufficiently rigorous and self-contained introduction to quantum theory,
 continuous variables, and quantum parameter estimation. We stress that quantum continuous variables are a mathematical tool, not a physical theory, and as such, they can be used to describe a wide range of phenomena, quantum light or optics being its most notable example.
    
An introduction to the theory of parameter estimation follows.  While the classical theory deals only with the statistics of measurement outcomes, and answers questions of attainability in the presence of statistical noise (with various properties that can affect the scaling of the precision with which one estimates  the parameter), quantum estimation addresses the problem of \textit{what} to measure, and imposes additional precision limits   due to to the fundamental probabilistic nature of quantum mechanics. 
Indeed, the quantum Fisher information (QFI) matrix, a key quantity in quantum estimation,  is defined an optimization of the classical Fisher information --a measure  for the amount of information relative to a set of parameters $\bm{\lambda}$ a system contains-- over all possible measurements, or POVMs.  Naturally, these areas pose very interesting questions regarding the very nature of statistics and the inherent probabilistic 
  aspect of quantum mechanics. In particular, we review some important results regarding Gaussian quantum parameter estimation, 
  a tool that can simplify enormously the computation of the QFI.
We use the case example of quantum illumination to confirm that the methods are able to reproduce known results with somewhat less effort than previous works.

The thesis contains a novel quantum sensing protocol, where we propose a  quantum-enhanced, idler-free sensing protocol to measure the response of a target object to the frequency of a probe in a noisy and lossy scenario.
{In our protocol, we consider a target with frequency-dependent reflectivity $\eta(\omega)$ embedded in a thermal bath. We aim at 
estimating the parameter $\lambda = \eta(\omega_2)-\eta(\omega_1)$, since it contains relevant information for different problems. 
For this, we employ as the resource a bi-frequency quantum state, since it is necessary to capture the relevant information about 
the parameter.}
Computing the quantum Fisher information $H$ relative to the parameter $\lambda$  in an assumed neighborhood  of $\lambda \sim 0$ for 
a two-mode squeezed state ($H_Q$), and a pair of coherent states ($H_C$), we show a quantum enhancement in the estimation of $\lambda$.
 This quantum enhancement grows with the mean reflectivity of the probed object, and is noise-resilient. We  derive explicit formulas 
 for the optimal observables, and propose an experimental scheme based on elementary quantum optical transformations. Furthermore, 
 our work opens the way to applications in both radar and medical imaging, in particular in the microwave domain.

Also oriented towards applications in microwave technology is the work we present 
 on the problem of distributing continuous-variable entanglement for the task of 
 implementing quantum teleportation in open-air. 

Microwave technology plays a central role in current wireless communications, including mobile communication and local area networks.
 The microwave range shows relevant advantages with respect to other frequencies in open-air transmission, such as low absorption 
 losses and low energy consumption, and in addition, it is the natural working frequency in superconducting quantum technologies. 
 Entanglement distribution between separate parties is at the core of secure quantum communications. Therefore, understanding its 
 limitations in realistic open-air settings, specially in the rather unexplored microwave regime, is crucial for transforming microwave
  quantum communications into a mainstream technology. Here, we investigate the feasibility of an open-air entanglement distribution 
  scheme with microwave two-mode squeezed states. First, we study the reach of direct entanglement transmission in open-air, obtaining 
  a maximum distance of approximately 500 meters with parameters feasible for state-of-the-art experiments. Subsequently, we adapt 
  entanglement distillation and entanglement swapping protocols to microwave technology in order to reduce the environment-induced 
  entanglement degradation. The employed entanglement distillation helps to increase quantum correlations in the short-distance 
  low-squeezing regime by up to $46\%$, and the reach of entanglement increases by $14\%$ with entanglement swapping. Importantly, 
  we compute the fidelity of a continuous-variable quantum teleportation protocol using open-air-distributed entanglement as a resource.
   Finally, we adapt this machinery to explore the limitations of quantum communication between satellites, where the impact of thermal 
   noise is substantially reduced and diffraction losses are dominant.


The thesis closes with a survey of propagating quantum microwaves and its applications as of today, both in communication and sensing. We argue the necessity for a 
 controllable quantum microwave interface, and explain why  is still in early stages. The results emphasize the need for a fully 
 functional toolbox and highlights potential research directions, including microwave quantum key distribution, quantum radar, 
 bath-system learning, and direct dark matter detection. By examining these applications, the paper underscores the wide range of 
 possibilities and future prospects in the field of quantum microwaves. For this, we construct a roadmap for future research lines 
 in the field of propagating quantum microwaves.  This chapter may be seen as an epilogue for the thesis, which functions both as a review of the state-of-the-art, and as an illustration of the wide reach of applications the 
future of quantum microwaves will open. 


\end{abstract}
\end{otherlanguage}






==> abstract/abstract-LongPT.tex <==
%!TEX root = ../dissertation.tex

\begin{otherlanguage}{portuguese}
\begin{abstract}
\abstractPortuguesePageNumber

A mecânica quântica é uma teoria física que tem beneficiado enormemente da comunidade matemática. Por um lado, a formulação da teoria de grupos de Hilbert, Weyl e outros, ajudou a refinar o rigor, clarificando alguns conceitos; por outro lado, e mais recentemente, a mecânica quântica começou a adotar ideias da teoria da informação através do trabalho de Shannon, Fisher e outros. Adoptando uma abordagem pragmática, e assumindo uma "coexistência pacífica" entre a mecânica quântica e a relatividade, podemos dizer que, uma vez demonstradas experimentalmente as principais previsões da mecânica quântica, em particular a existência de correlações para além das clássicas entre sistemas bipartidos, a teoria pode então ser utilizada. Mais especificamente, o rigor e uma perspetiva orientada para a informação, combinados, produzem uma teoria que é robusta e que pode começar a sair do estatuto experimental de prova de princípio para o domínio da aplicabilidade. É nesta altura que o \textit{tecnologia} quântico entra em jogo: A indústria começa a mostrar interesse no mundo quântico, numa batalha para capitalizar os resultados dos últimos cem anos, com o objetivo de resolver problemas da vida real com as novas ferramentas disponíveis, por vezes com uma abordagem exagerada que só o tempo, juntamente com um trabalho mais fundacional, provará ser oportuna.


As tecnologias quânticas são normalmente aplicadas em três categorias: computação, comunicação e deteção. O interesse industrial e político é justificado: a computação quântica tem um enorme potencial, não só na promessa de uma computação mais rápida e eficiente do que a clássica, mas também na simulação de sistemas quânticos; a comunicação quântica poderia trazer uma segurança sem precedentes devido à sua sensibilidade inerente
   A comunicação quântica poderá trazer uma segurança sem precedentes devido à sua sensibilidade inerente às escutas, suscitando o interesse da comunidade bancária. Alguns dos seus protocolos terão de ser incorporados na 
   A deteção quântica, que ultrapassa qualquer resolução classicamente possível, promete ideias de ficção científica como o radar quântico, a deteção direta de
    como o radar quântico, a deteção direta de matéria negra ou a exploração das propriedades quânticas da radiação cósmica de fundo em micro-ondas.


Nesta tese, damos a nossa contribuição teórica para uma dessas tecnologias quânticas emergentes: a propagação de micro-ondas quânticas. Esta plataforma encontra a sua motivação mais direta no facto de os circuitos supercondutores, uma das plataformas de computação quântica mais promissoras, que funcionam a uma temperatura criogénica (milikelvin), emitirem radiação que se enquadra na janela dos GHz.  Por conseguinte, se se pretender criar 
 uma rede de comunicação entre esses chips, faz sentido poder dispor de uma caixa de ferramentas tecnológicas capaz de explorar 
 o carácter quântico destes campos de propagação. Além disso, a janela de transparência atmosférica para as frequências de micro-ondas torna-as 
 torna-as candidatas adequadas para outras tarefas, como a comunicação quântica entre estações terrestres e satélites, ou para 
 deteção, incluindo, mas não se limitando a, radar quântico ou imagiologia. Os recentes avanços nos fotocontadores dedicados às micro-ondas 
 incentivam-nos a investigar mais este domínio de investigação relativamente novo, uma vez que a contagem de fotões fora de um campo eletromagnético 
 é um dos aspectos fundamentais de qualquer protocolo quântico, quer se trate de comunicação ou de deteção.


A primeira parte da tese é dedicada ao estabelecimento de uma introdução suficientemente rigorosa e autónoma à teoria quântica,
 variáveis contínuas e estimativa de parâmetros quânticos. Sublinhamos que as variáveis contínuas quânticas são uma ferramenta matemática e não uma teoria física e, como tal, podem ser utilizadas para descrever uma vasta gama de fenómenos, sendo a luz quântica ou a ótica o seu exemplo mais notável.


Segue-se uma introdução à teoria da estimativa de parâmetros.  Enquanto a teoria clássica lida apenas com as estatísticas dos resultados das medições e responde a questões de exequibilidade na presença de ruído estatístico (com várias propriedades que podem afetar o escalonamento da precisão com que se estima o parâmetro), a estimativa quântica aborda o problema do \textit{o que} medir e impõe limites de precisão adicionais devido à natureza probabilística fundamental da mecânica quântica. 
De facto, a matriz de informação quântica de Fisher (QFI), uma quantidade fundamental na estimativa quântica, é definida como uma otimização da informação clássica de Fisher - uma medida da quantidade de informação relativa a um conjunto de parâmetros $\bm{\lambda}$ que um sistema contém - sobre todas as medições possíveis, ou POVMs.  Naturalmente, estas áreas colocam questões muito interessantes relativamente à própria natureza da estatística e ao aspeto probabilístico inerente 
  probabilística da mecânica quântica. Em particular, analisamos alguns resultados importantes relativos à estimativa de parâmetros quânticos gaussianos, 
  uma ferramenta que pode simplificar enormemente o cálculo do QFI.
Utilizamos o exemplo do caso da iluminação quântica para confirmar que os métodos são capazes de reproduzir resultados conhecidos com um pouco menos de esforço do que os trabalhos anteriores.


A tese contém um novo protocolo de deteção quântica, em que propomos um protocolo de deteção quântica melhorado e sem ociosidade para medir a resposta de um objeto alvo à frequência de uma sonda num cenário ruidoso e com perdas.
{No nosso protocolo, consideramos um alvo com refletividade dependente da frequência $\eta(\omega)$ embebido num banho térmico. O nosso objetivo é 
estimar o parâmetro $\lambda = \eta(\omega_2)-\eta(\omega_1)$, uma vez que ele contém informações relevantes para diferentes problemas. 
Para isso, empregamos como recurso um estado quântico bifrequencial, já que ele é necessário para capturar as informações relevantes sobre o parâmetro. 
o parâmetro}.
Computando a informação quântica de Fisher $H$ relativa ao parâmetro $\lambda$ numa suposta vizinhança de $\lambda \sim 0$ para 
um estado espremido de dois modos ($H_Q$) e um par de estados coerentes ($H_C$), mostramos uma melhoria quântica na estimativa de $\lambda$.
 Esta melhoria quântica cresce com a refletividade média do objeto sondado e é resistente ao ruído. Derivamos fórmulas explícitas 
 para os observáveis óptimos, e propomos um esquema experimental baseado em transformações ópticas quânticas elementares. Além disso, 
 O nosso trabalho abre caminho a aplicações tanto em radar como em imagiologia médica, em particular no domínio das micro-ondas.

Também orientado para aplicações em tecnologia de micro-ondas é o trabalho que apresentamos 
 sobre o problema da distribuição do emaranhamento contínuo-variável para a tarefa de 
 para a tarefa de implementar o teletransporte quântico ao ar livre. 

A tecnologia de micro-ondas desempenha um papel central nas actuais comunicações sem fios, incluindo as comunicações móveis e as redes locais.
 A gama de micro-ondas apresenta vantagens relevantes em relação a outras frequências na transmissão ao ar livre, tais como baixas perdas por absorção 
 perdas por absorção e baixo consumo de energia e, além disso, é a frequência natural de trabalho nas tecnologias quânticas supercondutoras. 
 A distribuição do emaranhamento entre partes distintas está no centro das comunicações quânticas seguras. Por conseguinte, a compreensão das suas 
 Por conseguinte, a compreensão das suas limitações em cenários realistas ao ar livre, especialmente no regime de micro-ondas bastante inexplorado, é crucial para transformar as comunicações quânticas por micro-ondas numa tecnologia corrente.
  comunicações quânticas por micro-ondas numa tecnologia corrente. Aqui, investigamos a viabilidade de um esquema de distribuição de emaranhamento ao ar livre 
  com estados comprimidos de dois modos em micro-ondas. Em primeiro lugar, estudamos o alcance da transmissão direta do emaranhamento ao ar livre, obtendo 
  obtemos uma distância máxima de aproximadamente 500 metros com parâmetros viáveis para experiências de ponta. Posteriormente, adaptamos a 
  adaptamos os protocolos de destilação do emaranhamento e de troca do emaranhamento à tecnologia de micro-ondas para reduzir a degradação do emaranhamento induzida pelo ambiente. 
  degradação do emaranhamento induzida pelo ambiente. A destilação de emaranhamento empregue ajuda a aumentar as correlações quânticas no regime de curta distância 
  de curta distância até $46\%$, e o alcance do emaranhamento aumenta em $14\%$ com a troca de emaranhamento. Importante, 
  calculamos a fidelidade de um protocolo de teletransporte quântico contínuo e variável usando o emaranhamento distribuído ao ar livre como recurso.
   Finalmente, adaptamos esta maquinaria para explorar as limitações da comunicação quântica entre satélites, onde o impacto do ruído térmico 
   o impacto do ruído térmico é substancialmente reduzido e as perdas por difração são dominantes.


   A tese termina com uma análise da propagação de micro-ondas quânticas e das suas aplicações actuais, tanto na comunicação como na deteção. Defendemos a necessidade de uma interface 
 interface de micro-ondas quânticas controlável e explicamos porque é que ainda está numa fase inicial. Os resultados sublinham a necessidade de uma 
 Os resultados salientam a necessidade de uma caixa de ferramentas totalmente funcional e destacam potenciais direcções de investigação, incluindo a distribuição de chaves quânticas por micro-ondas, o radar quântico, 
 aprendizagem em sistema de banho e deteção direta de matéria negra. Ao examinar estas aplicações, o documento sublinha a vasta gama de 
 possibilidades e perspectivas futuras no domínio das micro-ondas quânticas. Para tal, construímos um roteiro para futuras linhas de investigação 
 no domínio da propagação das micro-ondas quânticas.  Este capítulo pode ser visto como um epílogo da tese, que funciona simultaneamente como uma revisão do estado da arte e como uma ilustração do vasto leque de aplicações que o 
aplicações que o futuro das micro-ondas quânticas abrirá. 



\end{abstract}
\end{otherlanguage}






==> acknowledgments/acknowledgments1.tex <==
%!TEX root = ../dissertation.tex

% Acknowledgments: This one is optional
\chapter*{Acknowledgments}
General thanks here:

Finally, I thank the support from the DP-PMI and FCT (Portugal) through scholarship PD/BD/135186/2017, as well as the EU H2020 Quantum Flagship project QMiCS (820505).






==> chapters/Communication.tex <==

%TEX root = ../dissertation.tex

\chapter{Communication}
\label{chapter:Communication}

\subsection{Quantum teleportation with CVs: FROM PAPER WITH TASIO}
Quantum teleportation is a quantum communication protocol which, in principle, allows to achieve perfect transfer of quantum information between two parties by means of previously shared entanglement, combined with local operations and classical communication. The protocol was first proposed in 1993 by Bennett and collaborators~\cite{Bennett1993}, as a way to take advantage of an entangled resource for the task of sending an unknown quantum state from one place to another, using discrete-variable quantum states. The original idea was simple, yet powerful: assuming that a maximally entangled, bipartite Bell state was shared between two parties (Alice and Bob) prior to the start of the protocol, Alice, in possession of some \textit{unknown} state $\ket{\psi}=\alpha\ket{0} + e^{i\beta}\sqrt{1-|\alpha|^2}\ket{1}$ couples her part of the Bell state to $\ket{\psi}$ by means of a Bell measurement, whose 2-bit output she communicates classically to Bob. Upon receiving the message, Bob performs a conditional unitary on his part of the shared Bell state, recovering $\ket{\psi}$ modulo a global phase in his location.

A year later, Vaidman extended the idea to the transmission of a CV state by means of a perfectly correlated (singular) position-momentum EPR state shared by Alice and Bob~\cite{Vaidman1994}. In 1998, Braunstein and Kimble~\cite{Braunstein1998} made this idea more realistic by relaxing the correlation condition to more experimentally-accessible states, such as finitely-squeezed states. Their protocol, known as the  Braunstein-Kimble protocol, was first realised by A. Furusawa and collaborators in 1998 in the optical domain~\cite{Furusawa1998}. We shall review the protocol here for convenience.

Kimble and Braunstein derived an expression for fidelity between an unknown state of a single mode Bosonic field and a teleported copy, when imperfect quantum entanglement is shared between the two parties. A generalization to a broadband version, where the modes have finite bandwidths, followed quite directly~\cite{Braunstein2005}. In the Braunstein-Kimble protocol, Alice and Bob share a TMSV state, which enables them to teleport the complete state of a single mode of the electromagnetic field, where two orthogonal field quadratures play the role of position and momentum. Shortly after, quantum teleportation of an unknown coherent state was demonstrated, showing an average fidelity (see Eq. \eqref{eq:Pure-PS-fidelity})  $\overline{F}=0.58 \pm 0.02$~\cite{Furusawa1998}, which beat the maximum classical fidelity of $\overline{F} = 0.5$ for Gaussian states~\cite{Braunstein2005, Serafini2017, Weedbrook2012}. Other works followed, where the Bell measurement of two orthogonal quadratures was replaced by photon-number difference and phase sum, and the question of an optimal quantum teleportation protocol depending on the entangled resource was raised~\cite{Milburn1999}. Subtraction of single photons from TMS states has been shown to enhance the fidelity of teleportation \cite{Opatrny2000, Cochrane2002}. We shall review here the Braunstein-Kimble protocol, replacing the Wigner function approach with its Fourier transform, the characteristic function. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
%\vspace{0.5cm}
\centering
\includegraphics[width=0.5\textwidth]{images/fig1.pdf}
\caption{Circuit representation of a CV microwave quantum teleportation protocol with Gaussian states. The entangled resource is harvested from two single-mode squeezed thermal states, generated from identical JPAs, which are then combined on a balanced beamsplitter. Assuming this state is generated by Alice, one of the modes has to be sent to Bob, represented here by the presence of antennae, in order for the two parties to share the entangled resource. Following this, Alice combined the target state to be teleported $|\psi_{\text{in}}\rangle_{\text{T}}$ with the mode of the entangled state she holds in a balanced beamsplitter, which is then subject to two homodyne detections, $x_\text{T}$ and $p_\text{A}$. The measurement results $\xi$ are communicated to Bob, who applies a displacement $\hat{D}(\xi)$ on his part of the entangled resource, resulting in the state $\rho^{\text{out}}_{\text{B}}$.}
\label{fig1}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The protocol goes as follows: 
\begin{enumerate}
\item Alice uses a 50:50 beam splitter to couple her part of the resource state $\rho_{AB}$ with an incoming unknown state $\rho^{\text{in}}_{T}$. The output Hilbert spaces of this beam splitter are labeled $A$ and $T$.
\item Alice performs two homodyne detections, where each of the local oscillator phases are set in order to measure photocurrents, whose differences are integrated over some time, and proportional to quadratures $\hat{x}_T := (\hat{x}_1  + \hat{x}_\text{in})/\sqrt{2}$ and $\hat{p}_A := (\hat{p}_1  - \hat{p}_\text{in})/\sqrt{2}$. She sends the outcomes $(x_T, p_A)$ to Bob via a classical communication channel.
\item Bob, upon reception of the signal $(x_T, p_A)$, performs a displacement $\hat{D}(\xi)$ to his part of $\rho_{AB}$, with $\xi := (x_T + ip_A)/\sqrt{2}$. The state at Bob's location is now, in average, closer to $\rho_{\text{in}}$ than what it would be if no entanglement was present in $\rho_{AB}$.
\end{enumerate}
For simplicity, we will denote $(x_T, p_A) = (x,p)$. The conditional state that Bob has after knowing the outcomes of Alice's homodyne measurements is
\begin{equation}
\rho_{B}(x,p) = \frac{1}{P_{B}(x,p)} \langle \Pi(x,p)| \rho_{T}^{\text{in}}\otimes \rho_{AB}|\Pi(x,p)\rangle_{TA},
\end{equation}
with $P_{B}(x,p) = \Tr_{B}\langle \Pi(x,p)| \rho_{\text{in}}\otimes \rho_{AB}|\Pi(x,p)\rangle_{TA}$, and 
\begin{equation}
\ket{\Pi(x,p)}_{TA} = \frac{1}{\sqrt{2\pi}}\int_\mathbbm{R}\diff y e^{ipy}\ket{x+y}_T\ket{y}_A,
\end{equation}
which is an element of the maximally entangled basis corresponding to Alice's Bell-like measurement. Now, this expectation value over the teleported ($T$) and the senders ($A$) modes is computed as 
\begin{widetext}
\begin{equation}
\langle \Pi(x,p)| \rho_{\text{in}}\otimes \rho_{AB}|\Pi(x,p)\rangle_{TA} = \frac{1}{2\pi}\int_{-\infty}^{\infty}\int_{-\infty}^{\infty} \diff y\diff y' e^{ip(y-y')}\langle x+y'|\rho_{\text{in}}|x+y\rangle_{T} \langle y'|\rho_{AB}| y\rangle_{A}.
\end{equation}
\end{widetext}
Once we have computed $\rho_{B}(x,p)$, we need to compute the outcoming state after the receiver applies the displacements, and average over all possible measurment outcomes
\begin{equation}
\rho_{B}^{\text{out}} = \int_{-\infty}^{\infty} \diff x \int_{-\infty}^{\infty} \diff p P_{B}(x,p)\hat{D}_{B}\left(\xi\right)\rho_{B}(x,p)\hat{D}^{\dagger}_{B}\left(\xi\right).
\end{equation}
As a measure of the quality of the protocol, one typically uses an overlap fidelity $F(\rho_\text{in}, \rho_\text{out}) = \Tr[\rho_{\text{in}}\rho_{\text{out}}]$, which corresponds to the Uhlmann fidelity $\left(\Tr[\sqrt{\sqrt{\rho_{\text{in}}}\rho_{\text{out}}\sqrt{\rho_{\text{in}}}}]\right)^{2}$ in the case when $\rho_{\text{in}}$ is pure. 

The figure of merit in quantum teleportation is the \textit{average} fidelity, which refers to the fact that we have averaged over all possible measurement outcomes,
\begin{equation}\label{eq:Pure-PS-fidelity}
\overline{F} = \Tr[\rho_{T}^{\text{in}}\rho_{B}^{\text{out}}].
\end{equation}
Sometimes it can be useful to have it written in terms of the CFs~\cite{Marian2006}:
\begin{equation}
\overline{F} =  \frac{1}{\pi}\int \diff ^{2}\beta \chi_{T}^{\text{in}}(-\beta)\chi_{B}^{\text{out}}(\beta),
\end{equation}
where the average over $(x,p)$ has already been performed in $\rho_{B}^{\text{out}}$.

If the resource state $\rho_{AB}$ is a Gaussian state with the covariance matrix given in Eq.~\eqref{eq:twoMode}, and the teleported state is a coherent state $|\alpha_{0}\rangle\langle\alpha_{0}|$, the average fidelity can be written as
\begin{equation}\label{eq:Gaussian-fidelity}
\overline{F} = \frac{1}{\sqrt{\det[\mathbbm{1}_{2} + \frac{1}{2}\Gamma]}},
\end{equation}
with $\Gamma \equiv (\sigma_Z \Sigma_A\sigma_Z + \Sigma_B -\sigma_Z \varepsilon_{AB}-\varepsilon_{AB}^\intercal\sigma_Z)$. Coherent states are typically the ones chosen to be teleported due to the ease of their experimental generation. In theory, the result of the average fidelity does not depend on the displacement $\alpha_{0}$; therefore, it will suffice to use an unknown coherent state for a demonstration of quantum teleportation. In experiments, however, the teleportation fidelity may depend on $\alpha_{0}$. 

It is also interesting to see the average fidelity of a process in which $k$ teleportation protocols are concatenated:
\begin{equation}
\overline{F}^{(k)} = \frac{1}{\sqrt{\det[\mathbbm{1}_{2} + \left(k-\frac{1}{2}\right)\Gamma)]}},
\end{equation}
assuming that, in each step, an entangled Gaussian resource with the covariance matrix that characterizes $\Gamma$ is used. 

Consider a symmetric covariance matrix with $\Sigma_{A}=\Sigma_{B}=\alpha\Id_{2}$ and $\varepsilon_{AB}=\gamma\sigma_{z}$. Then, we have $\Gamma = 2(\alpha-\gamma)\Id_{2}$ and $\tilde{\nu}_{-}=\alpha-\gamma$, which leads to
\begin{equation}\label{eq:Gaussian-fidelity}
\overline{F} = \frac{1}{1+\tilde{\nu}_{-}}.
\end{equation}
It is easy to check the two following limits for the average teleportation fidelity of an arbitrary coherent state: $\lim_{\tilde{\nu}_{-}\rightarrow 1} \overline{F} = 1/2$ and $\lim_{\tilde{\nu}_{-}\rightarrow 0} \overline{F} = 1$. The first limit corresponds to using no entanglement ($\tilde{\nu}_{-}\geq1$), and is interpreted as the `classical teleportation' threshold, meaning that any approach giving an average fidelity of 0.5 or less does not demonstrate quantum teleportation. The second limit corresponds to an idealized case of an infinite two-mode squeezing level ($\tilde{\nu}_{-}=0$), i.e., an EPR state, which realizes perfect quantum teleportation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\includegraphics[width=0.48\textwidth]{images/fig2.pdf}
\caption{Representation of an entanglement distribution protocol that uses antennae to efficiently transmit the quantum states into open-air, where photon losses and thermal noise effects are described with a beamsplitter with reflectivity $\eta_{\text{env}}$. We analyze two different scenarios: (a) Alice generates the entangled state, and attempts to share one of its modes with Bob by sending it through an noisy and lossy open-air channel that degrades the entanglement strength; (b) Charlie generates a two-mode entangled state, and sends one entngled mode to Alice and another to Bob. In this case, although both modes go through the same noisy and lossy channel, they travel half the distance as compared to the previous case.}
\label{fig2}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> chapters/QuantumIllumination.tex <==

\chapter{Quantum illumination between two cryogenic refrigerators}
\label{chapter:QuantumIllumination}
In this chapter we present some unpublished results regarding the realisation of quantum illumination between two cryogenic refrigerators. It represents a confirmation that the methods described in Chapter \ref{chapter:Estimation} are accurate, and useful, since we reproduce some well-known results from a slightly different approach. This chapter, hence, shall be used as a link to Chapter \ref{chapter:biFreq}, where proper novel results are presented.

\section{Quantum illumination as a parameter estimation problem in a nutshell}


\section{Quantum illumination with absorption losses}
Absorption losses in a homogeneous medium can be modeled as an array of $N$ `infinitesimal beams splitters'  spanned over length $L$, each of them with the same transmittivity per unit length $\mu_i$, where $i = 1, \ldots, N$.

Let's take two such beam splitters. Then, if they are embedded in the same environment, the combined transmittivity is $\tau^{(2)} =\tau_1 + \tau_2 - \tau_1\tau_2 $. Now, assuming that all transmittivities are equal, $\tau_i\equiv \tilde{\tau}=\mu L/N$ for all $i$, we get
\begin{equation}
\tau^{(2)}  = 2 \frac{\mu L}{N} \left( 1- \frac{\mu L}{2N} \right) =  2 \tilde{\tau} \left( 1- \frac{\tilde{\tau}}{2} \right).
\end{equation}
Treating this relation as an iterative equation, and using the logistic map, 
\begin{equation}
    x_{n+1} = r x_{n}(1-x_{n}),
\end{equation}
whose solution in the case $r=2$ is 
\begin{equation}
    x_{n} = \frac{1}{2} \left[ 1 - (1-2x_{0})^{2^{n}}\right],
\end{equation}
 we find that after $k$ iterations
\begin{equation}
\frac{\eta^{(k)}}{2}  =  \frac{1}{2} \left[ 1 - \left(1-\frac{\tilde{\eta} L}{N}\right)^{2^{k}}\right].
\end{equation}
Given that $N=2^{k}$, we take the limit on $k$, obtaining the following
\begin{equation}
\lim_{k\rightarrow\infty} \left(1-\frac{\tilde{\tau} L}{2^{k}}\right)^{2^{k}} = e^{-\tilde{\tau} L} \equiv e^{-\gamma},
\end{equation}
Therefore, the total reflectivity $\eta = 1-\tau$ of an array of infinitesimal beam-splitters, each having the same reflectivity per unit length is
\begin{equation}
\eta_{\text{loss}} = e^{-\gamma},
\end{equation}
and this shall represent a lossy medium in what follows.

Now, consider the situation depicted in  FIG. \ref{fig:2bs}. It is straightforward to compute the output $\hat{c}_2 = \sqrt{\eta_2 \left(1-\eta_1\right)}\hat{a}_1 + \sqrt{\eta_1 \eta_2}\hat{a}_2 + \sqrt{1-\eta_2}\hat{b}_2$. If we were to equate this to a single, effective beam splitter of reflectivity $\eta_\text{eff}$ mixing the same initial mode $\hat{a}_1$ with an effective bath $\hat{b}_\text{eff}$ it is clear that we must have: $\eta_\text{eff} = \eta_ 1 \eta_2 $ and $\hat{b}_\text{eff} = \hat{h}_\text{th} = \hat{a}_1 = \hat{b}_2$, such that $\langle \hat{h}^\dagger_\text{th} \hat{h}_\text{th} \rangle = N_\text{th}$. Therefore,  we set $\eta_\text{eff} = \eta e^{-\gamma}$ as the reflectivity of the combined beam splitter.

\begin{figure}
\centering
\includegraphics[width = 0.8\textwidth]{images/2bs.png}
\caption{bla bla}
\label{fig:2bs}
\end{figure}


As we have seen, QI can be presented as a quantum estimation problem, where the target's reflectivity $\eta$ is the parameter of interest.
Here, the model is as follows: the target object is represented by a low reflectivity beam splitter, which for simplicity introduces no phase. Additionally, absorption losses are modeled by a second beam splitter of reflectivity $\exp(-\gamma)$, where $\gamma := \alpha L$ is a dimensionless factor, and where $\alpha$ represents the loss per unit length, and $L$ is the linear total distance the signal travels. Note that this is a one dimensional-problem. As we have seen, the combination of two beam splitters of reflectivities $\eta_1$ and $\eta_2$ embedded in the \textit{same} environment (here a thermal state with $N_\text{th}$ photons) can be reduced to a single beam splitter with an effective reflectivity given by $\eta_\text{eff} = \eta_1\eta_2 $. In our case
\begin{equation}
\eta_\text{eff} = \eta e^{-\gamma}.
\label{eq:etaeff}
\end{equation}
 In the symplectic formalism, beam splitters  are represented by the  transformation
\begin{equation}
{S}_{\text{BS}}(x) = 
\left(
\begin{array}{cc}
x\Id_2 & \sqrt{1-x^2}\Id_2 \\
 -\sqrt{1-x^2}\Id_2 & x\Id_2
\end{array}
\right),
\label{eq:BS}
\end{equation}
where $x$ is the reflectivity.

QI can be seen as a procedure where a tripartite state of: thermal bath, signal, and idler, exhibiting bipartite entanglement between signal and idler, undergoes a transformation where the received state is bipartite and carries some dependence on $\eta$. An estimation of $\eta$ follows, performing some measurement and --perhaps-- post-processing the outcomes to construct an optimal estimator. Symbolically, an initial state characterized by a covariance matrix $\Sigma$ and a displacement vector $\vec{d}$ is mapped to an output state:
\begin{equation}
\left( \Sigma^\text{ABC}, \vec{d}^\text{ABC}\right) \mapsto \left( \Sigma^\text{DC}_\eta, \vec{d}^\text{DC}_\eta\right),
\end{equation}
where $A$, $B$, $C$ are the initial Hilbert spaces (bath, signal, and idler), and $D$ represents the Hilbert space where the reflected signal, mixed with the thermal noise, lives.

The classical strategy could be seen in a similar fashion, but not allowing for any non-classical correlations between any subsystems. In this case, the idler mode is clearly irrelevant, since it can't enhance the detection of $\eta$.  

\subsection{Quantum probe}
We use the following tripartite Gaussian state, which preserves the number of thermal photons and that is defined by a null displacement and a real covariance matrix given by
\begin{equation}
\Sigma=
\left(
\begin{array}{ccc}
 \Sigma_\text{A}  & 0 & 0  \\
 0 &  \Sigma_B &  \varepsilon_{BC}  \\
 0 &   \varepsilon_{BC}  &  \Sigma_C  
\end{array}
\right),
\label{eq:MikelState}
\end{equation}
where $\Sigma_\text{A} : = (1+ 2 N_\text{th})\Id$ is a thermal state with $N_\text{th}$ photons, $\Sigma_B = \left(1+2 N_\text{S}+2 N_\text{th}\right)\Id$, $\varepsilon_{BC} = 2 \sqrt{N_\text{S} (N_\text{S}+1)}\Sigma_{Z}$ are the correlations between subsystems $B$ and $C$, and $\Sigma_C = (1+2 N_\text{S})\Id$, where $\Id$ is the $2 \times 2$ identity matrix, and $\sigma_{Z}$ is the third Pauli matrix. In our setting, subsystem $C$ represents the idler mode, and $A$ and $B$ are the quantum entangled subsystems comprising the signal with photon number $N_\text{S}$ and the idler.
This covariance matrix satisfies the uncertainty principle, and as such represents a valid quantum  state. The motivation for using such a state is as follows: we want to have a state that has a \textit{fixed} thermal photon number $N_\text{th}$ while not exhibiting a shadow effect. Moreover, this state can also be obtained by mixing the signal part of a TMSV state with a modified thermal state with a $2\times 2$ covariance matrix $\left(1+2N_\text{th}(1-x)^{-1}\right)\Id$ via a beam splitter of reflectivity $x$, as already proposed in \cite{shapiroStory}.
The smaller symplectic eigenvalue  of the \textit{partially transposed} \cite{Adesso_2014} version  of the state in Eq. \eqref{eq:MikelState} is
\begin{widetext}
\begin{equation}
\tilde{\nu}_{-} = \sqrt{8 N_\text{S}^2-2 (2 N_\text{S}+N_\text{th}+1) \sqrt{4 N_\text{S} (N_\text{S}+1)+N_\text{th}^2}+4 N_\text{S} N_\text{th}+8 N_\text{S}+2 N_\text{th}^2+2 N_\text{th}+1}.
\end{equation}
\end{widetext}
The entanglement condition $\tilde{\nu}_{-} < 1$ reduces to $N_\text{S} > 0 \wedge N_\text{th} <1$. In Fig. \ref{fig:LogNeg} we plot the logarithmic negativity $E_\mathcal{N} := -\log_2 \tilde{\nu}_{-}$ as a function of the signal photon number $N_\text{S}$ for different $N_\text{th}$. In particular, $N_\text{th} = 0$ reproduces the negativity of the two-mode squeezed vacuum state, as expected. 
\begin{figure}
\centering
x\includegraphics[width=0.8\textwidth]{images/logNeg-Mikel.png}
\caption{Logarithmic negativity of the state in Eq. \eqref{eq:MikelState}}
\label{fig:LogNeg}
\end{figure}


The  thermal bath and the signal interact via Eq. \eqref{eq:BS} setting $x = \eta_\text{eff}$, while the idler mode is kept in a lossless delay line, represented by the identity operation. The total symplectic transformation for the full state is thus 
\begin{equation}
{S}_T = {S}_{\text{BS}}(\eta_\text{eff}) \oplus \Id.
\end{equation}
The transformed state is then represented by covariance matrix $\Sigma^\prime_\eta = {S}_T \Sigma_T {S}_T^\intercal$, which already carries the dependence on $\eta$, the parameter that we want to estimate using the Gaussian estimation techniques described above. Essentially, we want to discriminate between two channels: one where there is no object ($\eta = 0$) and another where there is a slightly reflective object ($\eta \ll 1$) \cite{Sanz_2017}. The goal is to show that the suggested state of Eq. \eqref{eq:MikelState} performs better than the classical optimal probe. The transmitted part of the signal is lost, which is implemented by removing the corresponding rows and columns of the covariance matrix. We call the received covariance matrix $\Sigma_\eta$, given by
\begin{equation}
\Sigma_\eta = 
\left(
\begin{array}{cc}
f\Id   & g\sigma_Z  \\
g\sigma_Z &  \Sigma_C
\end{array}
\right),
\end{equation}
where $f =1 +2N_\text{th} + 2N_\text{S} e^{-2\gamma}\eta^2$, $g = 2\sqrt{N_\text{S}\left(1+N_\text{S} \right)}e^{-\gamma}\eta$, and $\Sigma_C = 1 + 2N_\text{S}$. It can be seen that in the limit of infinite losses $\gamma \rightarrow \infty$ this state becomes an uncorrelated bath and an coherent idler state. 


We compute the quantum Fisher information relative to $\eta$ using the Gaussian formulas found in \cite{Safranek_2018, SafranekThesis}, working in the assumed neighborhood of $\eta \sim 0$. 
In order to avoid regularization schemes, the two symplectic eigenvalues of $\Sigma_\eta$ need to be larger than one. These conditions are equivalent to having $N_\text{S} > 0 \wedge N_\text{th} > 0$
The QFI is then found to be
\begin{equation}
 H_Q =  \frac{4 N_\text{S} e^{-2\gamma}(1+N_\text{S})}{1+2 N_\text{S} N_\text{th}+N_\text{S}+N_\text{th}}.
 \label{eq:HQ}
 \end{equation} 
As expected, when absorption losses tend to infinity, the QFI vanishes. It also vanishes for $N_\text{S}=0$, indicating that the protocol is free from shadow effects.
 \subsection{Classical probe}
 Here we use a coherent state as probe: $\ket{\psi} =\ket{\alpha}$, where we set $\alpha \in \mathbb{R}$ for simplicity. The expected photon number in this state is $\left| \alpha^2\right|$, and we set it equal to the signal photon number $N_\text{S}$ in the quantum state, for a matching-resources comparison.
The initial displacement vector of the total state (thermal bath, and signal) in the real basis is $\vec{d}_{0}^\intercal = (0,\sqrt{2}\alpha,0,0,0)$ which leads --after the interaction and the trace of the losses-- to  $\vec{d}_\eta^\intercal = (\sqrt{2}e^{-\gamma}\alpha\eta,0, 0,0)$.
We follow the same procedure as before, and compute the QFI $H_C$ for this state, inserting the displacement vector, and the covariance matrix in Eq. \eqref{eq:QFI}. We find 
\begin{equation}
H_C = \frac{4 e^{-2 \gamma } N_\text{S}}{2 N_\text{th}+1}
\label{eq:HC}
\end{equation}
In the next section, we compare the ratio $H_Q/ H_C$ to the one obtained in non-lossy QI.
\subsection{Comparison with quantum illumination}
In this section we compare our results to the ones obtained in \cite{Sanz_2017} for quantum illumination. The results are summarized in FIG. \ref{fig:comparison}. 
The gain $R \equiv H_Q/H_C$ of the lossy protocol turns out to be exactly that of the original, non lossy QI:

\begin{equation}
R = \frac{(1+N_\text{S}) (1+2 N_\text{th})}{1+2 N_\text{S} N_\text{th}+N_\text{S}+N_\text{th}}.
\end{equation}
This comes as no surprise, and it is actually a trivial result, coming from the additivity of the QFI. However, it proves that the methods are quite robust, and reproduce well-known results with a very straightforward calculation fashion. 

\begin{figure}
\centering
\includegraphics[width=0.7\textwidth]{images/QI.png}
\caption{Quantum Fisher information (QFI) ratio $H_Q/H_C$ for quantum illumination (QI) in the presence of losses (red) as a function of the signal photon number $N_\text{S}$ and the bath photon number $N_\text{th}$. In the low signal photon number and high noise photon number, the  protocol convergea to the 3dB limit: an overall factor of 2, represented by the plane $H_Q = 2H_C$. }
\label{fig:comparison}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.9\textwidth]{images/qi2d-Label.png}
\caption{Quantum Fisher information (QFI) ratio $H_Q/H_C$ for quantum illumination (QI) in the presence of losses as a function of the signal photon number $N_\text{S}$ for different bath photon number $N_\text{th}$. In the low signal photon number and high noise photon number, the  protocol convergea to the 3dB limit: an overall factor of 2, represented by the plane $H_Q = 2H_C$. }
\label{fig:2dQI}
\end{figure}



\section{Experimental scheme}
In this section, we give specific numbers to the lossy protocol in a cryogenic setting:
\begin{table}
\centering
\begin{tabular}{|l|c|c|}
\hline
Parameter &Symbol &Value\\
\hline
Losses per unit of length  &$\mu$ & $2.3\times 10^{-3} \text{km}^{-1}$\\
Emission aperture & $x$ & 10 cm\\
Reception aperture & $y$ & 10 cm\\
Signal wavelength in vacuum & $\lambda$  & 6 cm\\
Atmospheric temperature & $T$ &  300 K\\
Mean photon number & $N_\text{eff}$ & 1250\\
Squeezing parameter & $r$ &  1.32\\
Thermal photon number (signal) & $n$ & $8 \times 10^{-3}$ \\
\hline
\end{tabular}
\caption{Parameters for a terrestrial (1 atm of pressure, temperature of 300 K)  two-mode squeezed thermal state generated at a 50 mK cryostat, for a frequency of 5 GHz. These parameter values correspond to an Earth-based quantum teleportation scenario.}
\end{table} 
\begin{figure}[h!]
\centering
\includegraphics[width=0.8\textwidth]{images/fridges-2-labels.png}
\caption{Experimental scheme for the implementation of quantum illumination with losses between two cryogenic stations linked via a cryogenic cable.}
\end{figure}


==> chapters/Satellite.tex <==

\chapter{Satellites}
\label{chapter:satellites}



\subsection{Scaling and integration}
\label{subsec:qLAN}

The realization of a scalable QLAN for quantum communication is an important milestone for the implementation of distributed quantum computing and for quantum internet applications \cite{Awschalom2021}. Such a network should provide an all-to-all connectivity between distant superconducting quantum processors and simultaneously maintain quantum coherence of interactions, including a possibility for entanglement distribution. There has been already significant efforts towards QLAN implementation in the optical domain at telecom frequencies over fiber networks and in the free-space environment. However, after years of research efforts, microwave-to-optics transduction experiments still have not reached sufficiently good efficiencies. The latter remain on the order of $10^{-5}$ in the single-photon regime \cite{Mirhosseini2020} after accounting for post-selection probabilities or added noise photons. Furthermore, the materials compatibility of such converters with that of high-performance superconducting qubits also remains to be an outstanding problem. In order to avoid these problems, we consider a direct realization of microwave quantum networks by connecting spatially separated dilution refrigerators via a cryogenic microwave link \cite{Deppe2020}. This approach has two important advantages. First, microwaves are the natural frequency scale of superconducting quantum circuits and, therefore, frequency conversion losses trivially vanish in this scenario. Second, since superconducting quantum processors require cooling to millikelvin temperatures, the cryogenic requirements are reduced to the development of a suitable millikelvin interface between dilution fridges containing distant superconducting circuits. We have implemented this goal within the EU quantum Flagship project QMiCS together with  Oxford Instruments Nanotechnology Ltd. (OINT). Our cryogenic link with a total length of 6.6\,m reaches temperatures below $\SI{35}{\milli \kelvin}$ and connects a home-built dry dilution refrigerator with a commercial Triton500 dilution refrigerator from OINT \cite{Batey2009}, both dilution refrigerators reaching below $\SI{20}{\milli \kelvin}$. During the design phase of the cryogenic link, several unique features were incorporated. One of these is a cold ‘junction box’ (a cold network node (CNN)) at the mid-point of the link. In addition, due to the large radiative heat load from such a system -- \textit{i.e.}, two dilution refrigerators connected by a long cryogenic link -- the cooling power at the higher temperature stages is important. This radiative heat load can be reduced by adding multi-layer insulation, but in order to add significant cooling power, an extra Pulse Tube Refrigerator (PTR) or 1 K pot can be added to the CNN. Other unique design features will be discussed in further publications \cite{Renger2022}. An inter-fridge quantum communication channel within the cryolink is realized with a superconducting Niobium-Titanium coaxial cable with characteristic losses around $0.001$\,dB/m. The CNN furthermore allows to connect additional link arms and, therefore, enables scaling to a two-dimensional quantum area network. All integral parts for such a system were supplied commercially by OINT and could be supplied for future projects. This ensures straightforward scalability to longer distances and allows near-future implementation of distributed superconducting quantum computing platforms operating in the microwave regime \cite{Krinner2019,Magnard2020b}.


\begin{figure*}[t!]%[h]
\includegraphics[width=\linewidth]{images/network.pdf}
\caption{Idealized view of a section of an interconnected, large-scale quantum communications network that combines optical and microwave links. Two low-orbit satellites capable of performing QKD  protocols are optically connected to distant Earth-based stations. Quantum repeaters are then used to distribute the quantum resources throughout an entire network, making use of trusted quantum switches to choose which node(s) receive the quantum information. Locally, open-air microwave entanglement sources are used to entangle remote but relatively close stations (up to \SI{200}{\meter}), making use of the benefits of microwaves in open-air transmissions with unfavorable weather conditions (see Refs.~\cite{GonzalezRaya2022, Fesquet2022}), and a simplified version of a QLAN, where cryolinks are used to connect different cryogenic stations to perform local quantum communication or sensing experiments.}
\label{fig:network}
\end{figure*}


%\subsection{Quantum repeaters}
A key, elusive element for the task of scaling-up a quantum communication network to cover large distances is the quantum repeater (QR). In Figure \ref{fig:network} we show an idealized quantum network that makes use of QRs for long-range quantum communications. Classically, a repeater, in its simplest form, is a device sitting between two nodes of a network that receives an incoming noisy signal, measures it, reproduces a noiseless copy of the signal, and sends it to the other node. Given the fact that quantum information can't be cloned, this notion of repeater has to be revised. In order to be compatible with all the communication advantages the quantum realm offers, the most notable is its intrinsic security, quantum tomography is not a solution. This is because, in short, a receive-measure-send scheme would destroy any possible initial entanglement between the two active nodes. To overcome this, three generations of QRs have been identified, depending on the techniques they use to improve the communication rate between nodes, in a sophistication-increasing order. The first generation uses heralded entanglement generation (\textit{e.g.}, via entanglement swapping), heralded entanglement purification/distillation, or a mix of both. Essentially, these repeaters rely on the ability to perform Bell measurements and two-way classical communication between the nodes, which already pose a challenge in microwaves, as argued in Section \ref{subsec:detection}. Additionally, Gaussian entanglement distillation requires many copies of the state, which may not be possible in some scenarios. The following proposals for QRs all apply to the CV case. The approach of noiseless linear amplification, weak measurements, and postselection of Ref.~\cite{diCandia2015} have been conceived specifically for microwaves. A QR based on quantum scissors and non-deterministic, non-Gaussian entanglement swapping was proposed in Ref.~\cite{Seshadreesan2020}. The entanglement distillation, and swapping techniques discussed in Ref.~\cite{GonzalezRaya2022} will also prove relevant for this task. Single-shot QRs will be required at some point, but this requirement most likely will imply the need for microwave quantum memories~\cite{Wu2010,Kubo2012,Saito2013,Yin2013,Wenner2013,Flurin2014,Bao2021,Palomaki2013,Palomaki2013a}, as explained in Ref.~\cite{dias2020}. Still, models for quantum communications without quantum memories have been proposed \cite{Munro2012}. The second and third generations of quantum repeaters use classical and quantum error correction, respectively, to solve additional sources of imperfection in the incoming signal, and are still beyond current reach, to the best of our knowledge. Further, in the specific case of propagating quantum microwaves, much work needs to be done, both theoretically and experimentally to produce operative quantum repeaters, even of first generation.

%{\color{partner} VTT: can we hint at a possible implementation of a q. repeater for propagating quantum microwaves?}  %  Not really :D





==> chapters/conclusion.tex <==
%!TEX root = ../dissertation.tex

\chapter{Conclusion}
\label{chapter:conclusion}
Conclusion here\ldots 

\textbf{NOTE: 26 May 2023, do I really need this chapter?}
